On the abundance of intrinsically disordered proteins in the human proteome and its relation to diseases: there is no enrichment

Intrinsically disordered proteins are fascinating the community of protein science since the last decade, at least. There is a well-established line of research that intends to reveal the crucial role played by intrinsically disordered proteins (IDPs) in the development of human diseases. The main argument is that IDPs are differentially more present in groups of disease-related proteins. In this note we compare the frequency of disorder in human proteins, both disease-related and not. The frequency of disorder is comparable in the two sub-groups of proteins. Disorder is widespread in human proteins, but it is not a specific pre-requisite of proteins involved in the development of cancer, cardiovascular diseases, diabetes and neurodegenerative diseases. A tendency of cancer-related proteins to be statistically more disordered than the rest of human proteins is confirmed.

==> abstract.tex <==
\fontsize{9}{11}\selectfont 
Intrinsically disordered proteins are fascinating the community of protein science since the last decade, at least. There is a well-established line of research that intends to reveal the crucial role played by intrinsically disordered proteins (IDPs) in the development of human diseases. The main argument is that IDPs are differentially more present in groups of disease-related  proteins. In this note we compare the frequency of disorder in human proteins, both disease-related and not. The frequency of disorder is comparable in the two sub-groups of proteins. Disorder is widespread in human proteins, but it is not a specific pre-requisite of proteins involved in the development  of cancer, cardiovascular diseases, diabetes and neurodegenerative diseases. A tendency of cancer-related proteins to be statistically more disordered than the rest of human proteins is confirmed.

==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
 Antonio Deiana\\
  \fontsize{9}{11}\selectfont
  \textit{Physics Department, Sapienza University of Rome, P.le A. Moro 2, 00185 Rome, Italy}\\
  \fontsize{9}{11}\selectfont
  \textit{antonio.deiana@roma1.infn.it}\\[12pt]
  %
  \fontsize{11}{13}\selectfont
 Andrea Giansanti\\
  \fontsize{9}{11}\selectfont
  \textit{Physics Department, Sapienza University of Rome and INFN                                        sect. Roma1, P.le A. Moro 2, 00185 Rome, Italy}\\
  \fontsize{9}{11}\selectfont
  \textit{andrea.giansanti@roma1.infn.it}\\[12pt]
%
  % repeat previous group of commands here for further authors
}



==> keywords.tex <==
\fontsize{9}{11}\selectfont Natively unfolded proteins; intrinsic disorder; unfoldome; diseasome; cell signalling, cancer.


==> title.tex <==
% The Title is all in Uppercase
\newcommand{\mytitle}{\uppercase{On the abundance of intrinsically disordered proteins in the human proteome and its relation to diseases: there is no enrichment}\\
% The Subtitle should have initial letters capitalized
\fontsize{13}{15}\selectfont \textit{}
}


